Non-Exchangeable Conformal Language Generation with Nearest Neighbors

Quantifying uncertainty in automatically generated text is important for letting humans check potential hallucinations and making systems more reliable. Conformal prediction is an attractive framework to provide predictions imbued with statistical guarantees, however, its application to text generation is challenging since any i.i.d. assumptions are not realistic. In this paper, we bridge this gap by leveraging recent results on non-exchangeable conformal prediction, which still ensures bounds on coverage. The result, non-exchangeable conformal nucleus sampling, is a novel extension of the conformal prediction framework to generation based on nearest neighbors. Our method can be used post-hoc for an arbitrary model without extra training and supplies token-level, calibrated prediction sets equipped with statistical guarantees. Experiments in machine translation and language modeling show encouraging results in generation quality. By also producing tighter prediction sets with good coverage, we thus give a more theoretically principled way to perform sampling with conformal guarantees.

==> hallucination_section_dump.tex <==
\subsection{Detecting Hallucinations}\label{sec:detecting-hallucinations}

\begin{table}[htb]
    \centering
    \resizebox{\columnwidth}{!}{
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{rcccc}
    \toprule[0.05cm]
        Model & ATE & $\varnothing$ BF & FPR $\downarrow$ & FNR $\downarrow$ \\
        \midrule
        M2M100$_\text{(0.4B)}$ & \\
        M2M100$_\text{(1.2B)}$ & \\
        OPT$_\text{(350M)}$ & \\
        OPT$_\text{(1.3B)}$ & \\
         \bottomrule[0.05cm]
    \end{tabular}%
    }
    \caption{Results for hallucination experiments. Shown are the average treatment effect (ATE), the average Bayes factor obtained from the test in \cref{eq:bayes-factor} together with its false positive and false negative rate when faced with model hallucinations.}
    \label{tab:hallucination-results}
\end{table}

Lastly, we would like to investigate whether we can use the size of the calibrated prediction set as a possible indicator of hallucinations. Naturally, it is hard to evaluate this without knowing when hallucinations occur a priori. 
For this reason, we manipulate a model to encourage it to hallucinate based on recent mechanistic insights showing that during the hallucination process, the attention mechanism of the model ignores the source sentence \citep{berard2019naver, ji2023survey, guerreiro2023looking}. 
By restricting decoder attention to not access the source but only the generated prefix, we can force it to hallucinate. 
We can formalize this action as a causal intervention, allowing us to quantify the impact through the average treatment effect (ATE; \citealp{rubin1974estimating}).
Intuitively, the ATE quantifies the difference in a measured response variables between a treated cohort and a control group.
In our case, the treatment corresponds to generation without attention to the source, and the responsible variable to the observed prediction set size.
Given a prediction set $\mathcal{C}(y_t; y_{<t}, \bx)$ over possible continuations $y_t$ for an already generated prefix $y_{<t}$ given a source $\bx$, we can formalize the average treatment effect\footnote{For notional convenience, we assume for all sequences to be of the same length here.} as 

\begin{equation}\label{eq:ate}
    \displaystyle \text{ATE} \approx \frac{1}{TN}\sum_{i=1}^N\sum_{t=1}^T \big(S_t(\varnothing) - S_t(\bx)\big),
\end{equation}

\noindent where $S_t(\bx) \equiv |\mathcal{C}(y_t; y_{<t}, \bx)|$ and $S_t(\varnothing) \equiv |\mathcal{C}(y_t; y_{<t})|$ serve as shorthands for the size of the prediction sets.
In practice, we let the model generate first without any restrictions, and then feed the generated tokens back into the decoder, this time with no attention to the source.
We show results for our generation tasks in \cref{tab:hallucination-results}, showing that the ATE is positive, implying that---on average---the size of prediction sets increases when the model is forced to hallucinate.\\

More importantly, we would like to know whether we could use prediction set size as a potential detector of hallucinations. 
For this purpose, we repeat the procedure above on the calibration set to collect statistics about prediction set sizes per time step. 
Since we can think of set sizes as samples drawn from some distribution consisting of the sum of Bernoulli variables, we know that they are expected to be distributed according to $\mathcal{N}(\mu C, \sigma^2)$ due to the Central Limit Theorem, where $C$ denotes the size of the vocabulary.
We use this information to fit two normal distributions $p_t(\mu_t C, \sigma_t^2)$ and $q_t(m_t C, s_t^2)$ per time step to model hallucinatory and normal generation, respectively.
Given a generated sequence $\by$, we can construct a test based on the Bayes factor \citep{lodewyckx2011tutorial, morey2016philosophy} as 

\begin{equation}\label{eq:bayes-factor}
    \text{BF}_{10} = \frac{p(\mathcal{D}|\mathcal{M}_1)}{p(\mathcal{D}|\mathcal{M}_0)} \equiv \frac{\prod_{t=1}^T q_t\big(S_t(\varnothing) \big| m_t C, s_t^2\big)}{\prod_{t=1}^T p_t\big(S_t(\bx) \big| \mu_t C, \sigma_t^2\big)},
\end{equation}

where we compare the likelihood of observations $\mathcal{D}$ under to different models $\mathcal{M}_0$ and $\mathcal{M}_1$ corresponding to our two hypotheses.
Canonical decision thresholds can then help us to decide when to accept the null hypothesis $H_0$ ``the model is hallucinating'' and the alternative hypothesis $H_1$ ``the model is generating normally'', or when admit uncertainty and refrain from any decision. 
In our case, we take $\log \text{BF}_{10} \ge 3$ to accept $H_1$ and $\log \text{BF}_{10} \le -3$ to accept $H_0$ (corresponding to strong support for either hypothesis; \citealp{lodewyckx2011tutorial}).
Testing normally generated and hallucinated sequences on the test set with 
our fitted $q_t$ and $p_t$ allows us to report the average Bayes factor as well as Type I and II error rates for both cohorts in \cref{tab:hallucination-results}. 
